Annotating Data for Fine-Tuning a Neural Ranker? Current Active Learning Strategies are not Better than Random Selection

Search methods based on Pretrained Language Models (PLM) have demonstrated great effectiveness gains compared to statistical and early neural ranking models. However, fine-tuning PLM-based rankers requires a great amount of annotated training data. Annotating data involves a large manual effort and thus is expensive, especially in domain specific tasks. In this paper we investigate fine-tuning PLM-based rankers under limited training data and budget. We investigate two scenarios: fine-tuning a ranker from scratch, and domain adaptation starting with a ranker already fine-tuned on general data, and continuing fine-tuning on a target dataset. We observe a great variability in effectiveness when fine-tuning on different randomly selected subsets of training data. This suggests that it is possible to achieve effectiveness gains by actively selecting a subset of the training data that has the most positive effect on the rankers. This way, it would be possible to fine-tune effective PLM rankers at a reduced annotation budget. To investigate this, we adapt existing Active Learning (AL) strategies to the task of fine-tuning PLM rankers and investigate their effectiveness, also considering annotation and computational costs. Our extensive analysis shows that AL strategies do not significantly outperform random selection of training subsets in terms of effectiveness. We further find that gains provided by AL strategies come at the expense of more assessments (thus higher annotation costs) and AL strategies underperform random selection when comparing effectiveness given a fixed annotation cost. Our results highlight that ``optimal'' subsets of training data that provide high effectiveness at low annotation cost do exist, but current mainstream AL strategies applied to PLM rankers are not capable of identifying them.

==> sections/previous_notes.tex <==


\subsection{First motivational experiments: Variability in effectiveness for different training subsets}

\subsubsection{From scratch (MS Marco) for DR}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{pictures/msmarco_scatter_box/variance_traindata_size_scatter_ndcg@10_ordered_dr_marco.png}
    \caption{nDCG@10 effectiveness of training with different training dataset sizes for different number of epochs.}
    \label{fig:epochstrain}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{pictures/msmarco_scatter_box/variance_traindata_size_boxplot_ndcg@10_ordered_dr_marco.png}
    \caption{nDCG@10 effectiveness of training with different training dataset sizes for different number of epochs.}
    \label{fig:epochstrain}
\end{figure}

Look at scatterplot and boxplot of the variance within the trainings: We dont see a big variance here.


In the second plot \ref{fig:epochstrain} we see the effectiveness of the dense retrieval models trained on different training dataset sizes for different epochs. We see a major variability for small training dataset size (significant differences likely), little difference past 10k (any significant?).


\subsubsection{From scratch (MS Marco) for cross encoder ranking (BERT\textunderscore cat)}

Same experiments as for DR also for DistilBERT cross-encoder


\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{pictures/msmarco_scatter_box/variance_traindata_size_scatter_ndcg@10_ordered_bertcat_marco.png}
    \caption{MS Marco, BERT CAT, nDCG@10.}
    \label{fig:epochstrain}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{pictures/msmarco_scatter_box/variance_traindata_size_boxplot_ndcg@10_ordered_bertcat_marco.png}
    \caption{MS Marco, BERT CAT, nDCG@10.}
    \label{fig:epochstrain}
\end{figure}



\subsubsection{From scratch (MS Marco) for ColBERT}

Same experiments as for DR also for ColBERT (DistilBERT-based)


\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{pictures/msmarco_scatter_box/variance_traindata_size_scatter_ndcg@10_ordered_colbert_marco.png}
    \caption{MS Marco, ColBERT, nDCG@10.}
    \label{fig:epochstrain}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{pictures/msmarco_scatter_box/variance_traindata_size_boxplot_ndcg@10_ordered_colbert_marco.png}
    \caption{MS Marco, ColBERT, nDCG@10.}
    \label{fig:epochstrain}
\end{figure}

Look at scatterplot and boxplot of the variance within the trainings: For ColBERT similar picture as for BERT CAT, the variance is greater within the trainings and stay also bigger than for BERT CAT.

\section{Evaluation on TREC 2019 and TREC 2020}

\subsection{DR}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{pictures/msmarco_trec1920/variance_traindata_size_scatter_ndcg@10_ordered_trec2019_top1000_dr.png}
    \caption{MS Marco, DR, nDCG@10, TREC2019.}
    \label{fig:epochstrain}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{pictures/msmarco_trec1920/variance_traindata_size_boxplot_ndcg@10_ordered_trec2019_top1000_dr.png}
    \caption{MS Marco, DR, nDCG@10, TREC2019.}
    \label{fig:epochstrain}
\end{figure}

The variability for the dense retrieval evaluation of DR is greater than on MS Marco dev. Especially for the small training data sizes, one sees in the scatterplot that the samples with 5k and 10k training have similar performance and a great variability within the 5k trainings. The same holds for 20k training data size. Note also that the scale differences are much higher than in the scale for the MS Marco dev set. Therefore the variability in the performance across one training data size is between 4-10 points.



\subsection{BERT CAT}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{pictures/msmarco_trec1920/variance_traindata_size_scatter_ndcg@10_ordered_test_trec2019_top1000_bertcat.png}
    \caption{MS Marco, BERT CAT, nDCG@10, TREC2019 rerank BM25.}
    \label{fig:epochstrain}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{pictures/msmarco_trec1920/variance_traindata_size_boxplot_ndcg@10_ordered_test_trec2019_top1000_bertcat.png}
    \caption{MS Marco, BERT CAT, nDCG@10, TREC2019 rerank BM25.}
    \label{fig:epochstrain}
\end{figure}

The variability is especially big for 1k and 5k training sizes for BERT CAT. The performance of 5k and 10k samples is similar. The variability here is for 1k even 17 points for 10k 8 points. 


\subsection{ColBERT}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{pictures/msmarco_trec1920/variance_traindata_size_scatter_ndcg@10_ordered_test_top1000_6kdev_bm25rerank_colbert.png}
    \caption{MS Marco, ColBERT, nDCG@10, MSMArco dev rerank.}
    \label{fig:epochstrain}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{pictures/msmarco_trec1920/variance_traindata_size_boxplot_ndcg@10_ordered_test_top1000_6kdev_bm25rerank_colbert.png}
    \caption{MS Marco, ColBERT, nDCG@10, MS Marco dev rerank.}
    \label{fig:epochstrain}
\end{figure}

The variability here is for 1k and 5k is also there, but it is not so big, (look at the scale).

\section{Domain adaptation experiments}

\subsection{Training from scratch}

Training from scratch (DistilBERT) improves the performance but does not outperform BM25, nor TASB for Robust04 and not for Trec-Covid

Similar results in InPars \cite{bonifacio2022inpars} and GPL \cite{wang2021gpl}, in GPL they find that the starting checkpoint doesn't influence the overall performance of the model (start from DistilBERT or from DistilBERT trained on MS Marco).

\subsection{Training from pretrained model}

\subsubsection{Nfold cross validation training on Robust04}

Create on subsets of the test set of Robust04:
Take the description as query, take the positives as positives and the negatives as negatives. Dynamic negatives: More negatives than positives, to match the number and have a triple with one pos and one neg document, I use all negatives and add the positives as often, so that the every negative sample has a positive one.

First: no nfold cross-validation, only different training dataset sizes and their effectiveness: Sizes are 50, 100, 150, 200
The total number of test topics is 250, the difference between total and training size is used for testing!


\subsubsection{Robust 04: nfold training on subsets}

Randomly sample 50 queries from the test set. Create a training dataset from the qrels for these 50 queries, evaluate on the remaining 200 queries in the test set.

This leads to a training set with 50-60k samples. (Repeat positives to match all negatives).

From the training dataset constructed from these 50 queries, we sample subsets and then train the model on these subsets.

Subsets are sampled in the size 100,200,500,1k,5k.


\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{pictures/robust04_dr/variance_traindata_size_scatter_ndcg@10_ordered_dev_rob_subset50.png}
    \caption{Robust04 from TASB, variablity}
    \label{fig:epochstrain}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{pictures/robust04_dr/variance_traindata_size_boxplot_ndcg@10_ordered_dev_rob_subset50.png}
    \caption{Robust04 from TASB, variablity}
    \label{fig:epochstrain}
\end{figure}

Conclusions: You see that from 100-500 the DR model doesn't learn anything. But with 1k-10k the performance increases a lot. Not a lot of difference between 5k and 10k samples, within the subset size a lot of variability for 1k-10k, variability between 2-3 points.


\subsection{Conclusions from domain adaptation}

Domain adaptation with query generation does not work on top of TASB and CoCondenser. Also related work does not find that/ finds similar scores as we reach.

Knowledge distillation brings some gains, that you see an improvement, but not a lot. (around 1 point in nDCG@10 performance).

BUT: we see some outliers for Knowledge distillation
BUT: nfolds works well for Robust04, for TASB and for CoCondenser

Therefore the next steps will be:
\begin{itemize}
    \item Investigate the variability of the nfolds for robust 04 (implement n-fold cross validation and/or random sampling), do that tomorrow!
    \item Experiment on variability of Knowledge distillation (take BM25 negatives) (This training on ID, stopped for trec-covid, needs to be resumed)
    \item Same experiments with further training on TripClick, because here I have training data and I know that training improves the performance
    \item MS Marco for smaller training sizes, 100/200/500
\end{itemize}

Idea to train a domain specific model with question generation which improves on top of msmarco:

\begin{itemize}
    \item generate msmarco questions fitting to the target topics: 
    prompt tuning of a T5 model to generate from msmarco keyword queries, queries which fit to the style of questions in the target corpus
    \item QA model for documents and then scoring with crossencoder! here evidence from the annotation campaign
\end{itemize}


\subsubsection{Tripclick domain adaptation}

Did some experiments with TripClick, but it doesnt really learn something on smaller subsets (up to 5k).

\subsection{ESCI domain adaptation}

TASB zero shot reaches a 0.003 ndcg@10 on the qrels, training doesnt really improve the performance. I think more preprocessing of the text would be needed, and the winning approaches train a 4-class classfier, not a ranking model (ESCI classes).

Fixed the problems with ESCI

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{pictures/esci/variance_traindata_size_connected_ndcg@10_logFalse_test_top1000_test_dr.png}
    \caption{ESCI, incremental, DR, test.}
    \label{fig:escidr}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{pictures/esci/variance_traindata_size_connected_ndcg@10_logFalse_test_top1000_test_colbert.png}
    \caption{ESCI, incremental, ColBERT, test.}
    \label{fig:escicolbert}
\end{figure}


\section{Incrementally add training data}

Incrementally increase the training size.

\subsection{MS Marco}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{pictures/incremental/variance_traindata_size_connected_ndcg@10_logFalse_trec2019_top1000_marco_dr_ret.png}
    \caption{Marco DR, incremental, TREC 2019.}
    \label{fig:epochstrain}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{pictures/incremental/variance_traindata_size_connected_ndcg@10_logFals_marco_colbert2.png}
    \caption{Marco ColBERT, incremental.}
    \label{fig:epochstrain}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{pictures/incremental/variance_traindata_size_connected_ndcg@10_logFalse_marco_bertcat.png}
    \caption{Marco BERTCat, incremental.}
    \label{fig:epochstrain}
\end{figure}


\subsection{Robust04}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{pictures/incremental/variance_traindata_size_connected_ndcg@10_logFalse_description_top1000_rob_dr_ret.png}
    \caption{Robust04 DR, incremental.}
    \label{fig:epochstrain}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{pictures/incremental/variance_traindata_size_connected_ndcg@10_logFalse_rob_colbert.png}
    \caption{Robust04 ColBERT, incremental.}
    \label{fig:epochstrain}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{pictures/incremental/variance_traindata_size_connected_ndcg@10_logFalse_rob_bertcat.png}
    \caption{Robust04 BERTCAT, incremental.}
    \label{fig:epochstrain}
\end{figure}



